Improved Throughput for All-or-Nothing Multicommodity Flows with Arbitrary Demands

Throughput is a main performance objective in communication networks. This paper considers a fundamental maximum throughput routing problem -- the all-or-nothing multicommodity flow (ANF) problem -- in arbitrary directed graphs and in the practically relevant but challenging setting where demands can be (much) larger than the edge capacities. Hence, in addition to assigning requests to valid flows for each routed commodity, an admission control mechanism is required which prevents overloading the network when routing commodities. We make several contributions. On the theoretical side we obtain substantially improved bi-criteria approximation algorithms for this NP-hard problem. We present two non-trivial linear programming relaxations and show how to convert their fractional solutions into integer solutions via randomized rounding. One is an exponential-size formulation (solvable in polynomial time using a separation oracle) that considers a "packing" view and allows a more flexible approach, while the other is a compact (polynomial-size) edge-flow formulation that allows for easy solving via standard LP solvers. We obtain a polynomial-time randomized algorithm that yields an arbitrarily good approximation on the weighted throughput, while violating the edge capacity constraints by only a small multiplicative factor. We also describe a deterministic rounding algorithm by derandomization, using the method of pessimistic estimators. We complement our theoretical results with a proof of concept empirical evaluation.

==> constant-violation-result.tex <==
\newcommand{\scal}{\ensuremath{c}}
\newcommand{\fscal}{\ensuremath{\tilde{f}'}}
\newcommand{\cscal}{\ensuremath{c'}}
\newcommand{\wscal}{\ensuremath{\Expec[w'_{ALG}]}} %

Above, (deterministic) approximations for the ANF were given that achieve a throughput of $\alpha \geq 1/3$ and violate edge capacities by the logarithmic term $\beta \in \mathcal{O}(\log n)$. In the following, we discuss trading off the respective approximation objectives. Specifically, we show that by scaling the capacities by a factor $0 < \scal \leq 1$, a $(\scal \cdot \alpha, \scal \cdot \beta)$-approximation can be obtained whenever the achieved throughput is not rendered too small. 

We first discuss the changes pertaining to the randomized Algorithm~\ref{alg:randomrounding}. After pruning requests that cannot be embedded and computing the LP in Line~2, the flow values are scaled by the factor $0 < \scal  \leq 1$ by setting $\fscal_i = \scal \cdot \tilde{f}_i$ and $\fscal_{i,e} = \scal \cdot \tilde{f}_{i,e}$.
 After scaling the flows, the scaled solution is valid with respect to the scaled down capacities $\cscal_e = \scal \cdot c_e$ and demands $d'_i=\scal\cdot d_i$, and achieves exactly a $\scal$-factor of the original solution's throughput: i.e., $w'_{ALG}=\scal \cdot w_{ALG}$ and $\wscal = \scal \cdot \Expec[w_{ALG}]$ holds. 
 
Notably, the rescaled solution may not route all commodities fully with respect to the new capacities. However, the analysis laid out in Theorem~\ref{theorem:throughput} only requires that $w_{\max} \leq \wscal$ holds. Assuming this condition to hold, the subsequent analyses  remain valid and by randomized rounding a $(\alpha, \beta)$-approximate solution regarding to the scaled down capacities and scaled down flows is obtained. Reinterpreting the scaled solution with respect to the \emph{original} capacities and the originally achieved LP throughput, it is easy to check that the obtained solution is indeed $(\scal \cdot \alpha, \scal \cdot \beta)$-approximate. As the derandomization result of Section~\ref{sec:derandomization} is purely based on the analysis of Section~\ref{sec:randomized-algorithm}, it also carries over. Given our above argument, we state the following without proof:

\begin{theorem}
	By scaling the flows by a factor $0 < \scal \leq 1$, a deterministic $(\scal \cdot \alpha, \scal \cdot \beta)$-approximation for the ANF is obtained with $\alpha = 1 - 2/3 \cdot \sqrt{w_{\max}/w_{LP}} \geq 1/3$ and $\beta = 1 + 3\log n$ for $n \geq 9$ as long as $\scal \cdot w_{LP} \geq w_{\max}$ holds.  
\end{theorem}

Assuming that all commodities can be routed using only a $\Theta(\log n)$-fraction of the capacities, the following corollary is obtained:

\begin{corollary}
	Assuming that all commodities are routable using an $\Theta(\log n)$ fraction of the original capacities in the absence of other commodities, then a $(1/\Theta(\log n), \Theta(1))$-approximate solution can be computed by scaling the flows by $1/\Theta(\log n)$ before rounding.
\end{corollary}

